The Art, Science, and Engineering of Fuzzing: A Survey

Among the many software vulnerability discovery techniques available today, fuzzing has remained highly popular due to its conceptual simplicity, its low barrier to deployment, and its vast amount of empirical evidence in discovering real-world software vulnerabilities. At a high level, fuzzing refers to a process of repeatedly running a program with generated inputs that may be syntactically or semantically malformed. While researchers and practitioners alike have invested a large and diverse effort towards improving fuzzing in recent years, this surge of work has also made it difficult to gain a comprehensive and coherent view of fuzzing. To help preserve and bring coherence to the vast literature of fuzzing, this paper presents a unified, general-purpose model of fuzzing together with a taxonomy of the current fuzzing literature. We methodically explore the design decisions at every stage of our model fuzzer by surveying the related literature and innovations in the art, science, and engineering that make modern-day fuzzers effective.

==> ack.tex <==
%
\section*{Acknowledgment}

The authors would like to thank...

developers of BFF for pointing out a mistake in an earlier draft %

%
%
%
%


==> figs/taxonomy.tex <==
{
\footnotesize
\usetikzlibrary{shapes,positioning}
\usetikzlibrary{matrix}
\usetikzlibrary{calc}
\newsavebox{\fuzzerstab}
\sbox{\fuzzerstab}{
\tabulinesep=1.2mm
\begin{tabu}{ l|l|[2pt]X[c] X[c] }
  \multicolumn{2}{c|[2pt]}{\multirow{2}{*}{}}
 & \multicolumn{2}{c}{Input Generation Methods} \\
\cline{3-4}
%
   \multicolumn{2}{c|[2pt]}{\vphantom{}}
 & \multicolumn{1}{c|}{Model-based Generation}
 & \multicolumn{1}{c}{Model-less Generation} \\
%
\tabucline[2pt]{-}
  \multirow{2}{*}{\rotatebox[origin=c]{90}{Granularity}}
 &
  \multirow{1}{*}{\rotatebox[origin=c]{90}{Black-Box}}
          & \vspace{6.0cm}
          & \\
\tabucline[1pt off 2pt]{2-4}
 &
  \multirow{1}{*}{\rotatebox[origin=c]{90}{Grey-Box}}
          & \vspace{4.0cm}
          & \\[0.05cm]
\tabucline[1pt off 2pt]{2-4}
%
 &
  \multirow{1}{*}{\rotatebox[origin=c]{90}{White-Box}}
  & \multicolumn{2}{c}{\parbox{3cm}{\vspace{2.6cm}}} \\
\end{tabu}
}

\begin{tikzpicture}[
    every node/.style={inner sep=0,outer sep=0},
    every label/.style={font=\bf\scriptsize}
  ]
\node (fuzzers) [shape=rectangle] {\usebox{\fuzzerstab}};
\tikzstyle{fuzzerbox} = [draw=gray,rounded corners,fill=white,text opacity=1,fill opacity=0.2,thick,inner sep=5pt];
\matrix[anchor=west,baseline=(current bounding box.north)] at (-6.50cm, 0.95) {
  \node[fuzzerbox,fill=green!30, label={[xshift=-6.55cm,yshift=0.1cm,align=right]above:General Purpose},text width=14.8cm] {
    \begin{tikzpicture}
      \node[text width=7.0cm] (bbgeneral) {
        antiparser~\cite{antiparser},
        Dharma~\cite{dharma},
        Neural\-Fuzzer~\cite{neural}, % Neural-Net
        Peach~\cite{peachfuzz}, % basic?
        Sulley~\cite{sulley}, % Http? Network; + File?
        Tavor~\cite{tavor} % generic; User-given model
      };
      \node[text width=6.0cm,right=1.1cm of bbgeneral] {
        GPF~\cite{gpf}, % Basic?
        Hodor~\cite{hodor}, % General-use, text
        Radamsa~\cite{radamsa} % ??
      };
    \end{tikzpicture}
  };\\
  \node[fuzzerbox,fill=blue!30,label={[xshift=-6.84cm,yshift=0.1cm,align=right]above:File Format},text width=14.8cm] at (0, -1.1) {
    \begin{tikzpicture}
      \node[text width=7.0cm] (bbfile) {
        cross\_fuzz~\cite{crossfuzz}, % DOM, Browser
        DOMFuzz~\cite{funfuzz},
        Fuzzbox~\cite{david:blackhat2008}, % multi-codec media
        IFuzzer~\cite{veggalam:esorics2016},
        jsfunfuzz~\cite{funfuzz},
        LangFuzz~\cite{holler:usec2012}, % Javascript, Browser
        Melkor~\cite{melkor}, % ELF, (Kernel or binutils?)
        Nduja~\cite{valotta:2012},
        ref\_fuzz~\cite{reffuzz},
        SPIKEfile~\cite{sutton:blackhat2005}
      };
      \node[text width=6.5cm,right=1.1cm of bbfile] {
        BFF~\cite{bff}, % Basic?
        certfuzz~\cite{certfuzz},
        FileFuzz~\cite{filefuzz},
        FOE~\cite{foe}, % Basic?
        MiniFuzz~\cite{minifuzz}, % basic
        zzuf~\cite{zzuf} % Bitflip
      };
    \end{tikzpicture}
  };\\
  \node[fuzzerbox,fill=yellow!50,label={[xshift=-2.35cm,yshift=0.1cm,align=right]above:Network Protocol},text width=6.5cm] (bbnet) at (0, -1.2) {
    \begin{tikzpicture}
      \node[text width=6.5cm] {
        Autodaf\'{e}~\cite{vuagnoux:2005}, % Block-based, File, Network
        KameleonFuzz~\cite{duchene:codaspy2014},
        KiF~\cite{abdelnur:iptcomm2007},\\
        llfuzzer~\cite{llfuzzer}, % NFC
        LZFuzz~\cite{bratus:2008}, % Protocol
        PROTOS~\cite{kaksonen:2001},\\
        PULSAR~\cite{gascon:seccomm:2015}, % network fuzzer, Model Inference
        SPIKE~\cite{spike}, % Block-based ??, Network?
        SNOOZE~\cite{banks:2006},
        T-Fuzz~\cite{johansson:icst2014},
        tlsfuzzer~\cite{tlsfuzzer} % TLS
      };
      %\node[text width=6.0cm,right=1.1cm of bbnet] {
      %};
    \end{tikzpicture}
  };
  \node[fuzzerbox,fill=magenta!60,label={[xshift=-3.20cm,yshift=0.1cm,align=right]above:UI},right=8.1cm of bbnet] at (0, -0.75){
    \begin{tikzpicture}
     \node[text width=6.7cm,xshift=-0.9cm] (bmutetc) {
        Monkey~\cite{monkey},
        Orangutan~\cite{orangutan}
      };
    \end{tikzpicture}
  };\\
  \node[fuzzerbox,fill=red!30,label={[xshift=-2.9cm,yshift=0.1cm,align=right]above:Kernel}] (blackkernel) at (0, -0.75){
    \begin{tikzpicture}
      \node[text width=6.5cm] (bkernel) {
        fsfuzzer~\cite{fsfuzzer},
        KernelFuzzer~\cite{kernelfuzzer},
        Trinity~\cite{trinity}
      };
    \end{tikzpicture}
  };\\
  \node[fuzzerbox,fill=blue!30,label={[xshift=-6.7cm,yshift=0.1cm,align=left]above:File Format},text width=14.8cm] (greyfile) at (0, -1.2) {
    \begin{tikzpicture}
      \node[text width=2.0cm] (greyfileempty) { };
      \node[text width=4.5cm,right=0.0cm of greyfileempty] (greymodelfile) {
        Choronzon~\cite{sialveras:zeronights2015},
        Nightmare~\cite{nightmare}, % distributed
        QuickFuzz~\cite{grieco:2016} % various formats
      };
      \node[text width=3.3cm,right=1.6cm of greymodelfile,text height=0.2cm,text depth=0.3cm] (greysrcbin) {
        AFL~\cite{aflfuzz}, % Genetic
        AFLFast~\cite{boehme:ccs2016}, % Genetic, Scheduling
      };
      \node[text width=4.0cm,right=0.05cm of greysrcbin,text height=0.2cm,text depth=0.3cm] {
        GRR~\cite{grr}, % emulation
        honggfuzz~\cite{honggfuzz},\\ % Hard-ware support
        Mamba~\cite{seagle:2012}
      };
    \end{tikzpicture}
  };\\
  \node[fuzzerbox,fill=red!30,label={[xshift=-2.9cm,yshift=0.1cm,align=right]above:Kernel},xshift=3.4cm,below=0.0cm of bmutetc] (greykernel) at (0, -0.4) {
    \begin{tikzpicture}
      \node[text width=6.5cm,text height=0.30cm,text depth=0.2cm] {
        syzkaller~\cite{syzkaller},~~
        Triforce Linux Syscall Fuzzer~\cite{triforce}
      };
    \end{tikzpicture}
  };\\
  \node[fuzzerbox,fill=green!30,label={[xshift=6.55cm,yshift=-0.1cm,align=right]below:General Purpose},text width=14.8cm] (greygeneral) at (0, -0.8) {
    \begin{tikzpicture}
      \node[text width=6.5cm] (greygengeneral){
        Randoop~\cite{pacheco:icse2007},\\ % API
        Sidewinder~\cite{shawn:blackhat2006} % Genetic % Need full CFG -> White-box??, No specific target (maybe network)
      };
      \node[text width=6cm,xshift=-0.2cm,right=1.8cm of greygengeneral] {
        LibFuzzer~\cite{libfuzzer}, % In-process
        ossfuzz~\cite{ossfuzz}, % In-process
        ~~EFS~\cite{demott:blackhat2007} % Genetic
      };
    \end{tikzpicture}
  };\\
};
\node[fuzzerbox,fill opacity=0,densely dashed,label={[xshift=-0.1cm,yshift=-0.0cm,align=right]left:Source\\Based},below=0.8cm of greygeneral,xshift=-4.50cm,text width=5.5cm,text height=0.2cm] (whitesource) {
  BuzzFuzz~\cite{ganesh:icse2009},
  Dowser~\cite{haller:usec2013},
  jFuzz~\cite{jayaraman:2009}
};
\node[fuzzerbox,fill opacity=0.1, fill=black, densely
dashed,label={[xshift=-0.1cm,yshift=-0.0cm,align=right]left:Binary\\Based},below=0.2cm
of whitesource,xshift=0.00cm,text width=5.5cm,text height=0.2cm] (whitebinary) {
  Driller~\cite{stephens:ndss2016},
  FuzzBALL~\cite{babic:issta2011,lorenzo:asplos2012,caselden:eecs-2013-85},
  Mayhem~\cite{cha:oakland2012,avgerinos:icse2014},
  MoWF~\cite{pham:ase2016},
  SAGE~\cite{godefroid:ndss2008, godefroid:pldi2008},
  SmartFuzz~\cite{molnar:2009},
  TaintScope~\cite{wang:oakland2010}
};
% \node[text width=4.0cm,below=0.8cm of greyetc,xshift=1.2cm] (whitesource) {
%\draw[densely dashed,rounded corners] ($(greykernel.west) + (2cm, 0.3cm)$) --
%                                      ($(greykernel.west) + (0.1cm, 0.3cm) $) --
%                                      ($(whitesource.west) + (-0.1cm, -0.6cm)$) --
%                                      ($(whitesource.east) + (-0.1cm, -0.6cm)$);
\draw[densely dashed,rounded corners,fill opacity=0.1,fill=black]
    ($(greyfile.north) + (-5.5cm, -0.1cm)$) --
    ($(greyfile.north) + (7.5cm, -0.1cm) $) --
    ($(greygeneral.south) + (7.5cm, 0.1cm)$) --
    ($(greygeneral.south) + (4.1cm, 0.1cm)$) --
    ($(greygeneral.north) + (4.1cm, 0.2cm)$) --
    ($(greygeneral.north) + (-5.5cm, 0.2cm)$) --
    cycle;
\node[rotate=-90,
      right=of greyfile,
      xshift=0.9cm,
      yshift=-0.7cm,
      align=left,
      font=\bf] {\scriptsize Binary\\\scriptsize Based};
\node[fuzzerbox,
      fill opacity=0.1,
      fill=white,
      densely dashed,
      label={[xshift=-0.2cm,yshift=0cm,align=right]left:Source\\Based},
      left=0.0cm of greykernel,
      xshift=2.05cm,
      yshift=-0.8cm,
      text width=1.58cm,
      text height=1.8cm] { };
%\node[fuzzerbox,
%      fill opacity=0.1,
%      fill=black,
%      densely dashed,
%      label={[xshift=0.0cm,yshift=0.05cm,align=left]above:Binary Based},
%      right=0.0cm of greyfile,
%      xshift=-13.00cm,
%      yshift=-0.5cm,
%      text width=3.9cm,
%      text height=1.8cm] { };
%%%%%
\node[fuzzerbox,
      fill opacity=0.1,
      fill=white,
      densely dashed,
      label={[xshift=0.0cm,yshift=0.1cm,align=left]above:Source Based},
      right=0.0cm of greyfile,
      xshift=-6.9cm,
      yshift=-1.3cm,
      text width=2.9cm,
      text height=3.3cm] { };
%\node[fuzzerbox,
%      fill opacity=0.1,
%      fill=black,
%      densely dashed,
%      label={[xshift=2.3cm,yshift=-0.1cm,align=left,rotate=0]below:Binary Based},
%      right=0.0cm of greyfile,
%      xshift=-7.00cm,
%      yshift=-0.00cm,
%      text width=6.0cm,
%      text height=0.4cm] { };
\end{tikzpicture}
}


==> setup.tex <==
\section{Experimental Setup}\label{sec:setup}

%

To raise research questions, we first build our test suite, and run a
variety of experiments on it. The test suite makes use of a set of
popular programs on Debian Jessie that can parse audio, image, or
video files from a command line. To collect such programs, we
performed the following steps.

First, we enumerated all the packages in Debian Jessie (mirrored on 09/13/2016)
that include at least one program satisfying the following conditions: (1) the
program should be written in either C or C++; (2) the program can process audio,
image, or video files; (3) we can run the program with a command line; and (4)
the program does not have a GUI. To achieve this, we used the \texttt{debtags}
utility with the following commands.
%
\begin{lstlisting}[language=bash,basicstyle=\ttfamily\footnotesize,showstringspaces=false]
debtags search "(! interface::x11) \
             && (works-with::audio \
                 || works-with::image \
                 || works-with::video) \
             && (implemented-in::c \
                 || implemented-in:c++) \
             && interface::commandline \
             && role::program"
\end{lstlisting}

Second, we sorted all the packages we obtained from the first step by their
popularity~\cite{debpopcon}. We then downloaded top 50 popular packages from the
list, and picked one binary from each of the packages.
%
Finally, we ran AFL~\cite{aflfuzz} (version 2.35b) for 24 hours on each of the
50 executables, and selected top 10 popular programs that produce at least one
reproducible crash. Table~\ref{tab:dataset} summarizes a list of programs that
we selected.

\begin{table}[ht]
  \centering
  \begin{tabu}{ l X[l] r r }
    \textbf{Program} & \textbf{Package} & \textbf{\# of Crashes} &
    \textbf{Rank}\\
  \tabucline[2pt]{-}
  gs & ghostscript & 5 & 1 \\
  fig2dev & transfig & 400 & 4 \\
  dvdauthor & dvdauthor & 1 & 5 \\
  ufraw-batch & ufraw-batch & 16 & 6 \\
  gnuplot-nox & gnuplot-nox & 1 & 8 \\
  wrestool & icoutils & 243 & 10 \\
  dcraw & dcraw & 29 & 15 \\
  wvunpack & wavpack & 112 & 16 \\
  sndfile-play & sndfile-programs & 107 & 26 \\
  ocrad & ocrad & 14 & 33 \\
  \end{tabu}
  \caption{A list of programs used in our experiments.}
  \label{tab:dataset}
\end{table}

%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%

%
%

